Any2Building: Unifying Point Clouds and Images for Building Reconstruction via Shared Spatial Queries

Abstracting structured buildings from limited observations is essential for 3D urban modeling and digital twins. Partial point clouds and overhead images of the same building provide incomplete 3D surface measurements and visual cues to its footprint, roof geometry, and rooftop structures, respectively. This motivates a unified framework that aligns geometric and visual cues in 3D and reconstructs buildings from either or both modalities. Building on this connection, we present Any2Building, a unified model for Level of Detail 2 (LoD2) building reconstruction from partial point clouds, overhead images, or both, with optional coarse geometric priors. At its core is an occupancy-grounded shared spatial queries representation that organizes available observations within a common 3D grid. Supervised by complete building surface voxels, these queries connect observational evidence to target geometry, enabling a shared generator to learn structural priors across tasks and providing spatial guidance for recovering missing structure. A trained voxel conditional surface-generation and low-poly remeshing pipeline then converts the predicted structure into compact LoD2 building models. To support this framework, we introduce BuildingWorld-Image, comprising approximately one million paired samples of partial point clouds, overhead images, and LoD2 building models across 18 cities. Experiments on multiple benchmarks demonstrate that Any2Building outperforms existing methods in geometric reconstruction accuracy across unimodal and multimodal point-cloud completion, single-image building generation, and prior-assisted generation, while maintaining detailed and robust recovery when point cloud input modality is degraded.

==> tables/completion_combined.tex <==
% % \begin{table}[!t]
% % \centering
% % \caption{\textbf{Unimodal and multimodal point-cloud completion.} The upper group uses partial points alone; the lower group evaluates sparser partial observations, with paired images available to multimodal methods. P: points; I: image. CD/EMD $\times10^3$. Metrics without the PC prefix are evaluated on the final low-poly
% % meshes. PC CD-L1 and PC-F are evaluated on the outputs before surface generation and low-poly reconstruction.}
% % \label{tab:completion-combined}
% % \label{tab:supp-selected}
% % \label{tab:supp-multimodal}
% % \footnotesize
% % \setlength{\tabcolsep}{3pt}
% % \resizebox{\columnwidth}{!}{%
% % \begin{tabular}{@{}lccccccccc@{}}
% % \toprule
% % Method & Input & CD-L1 $\downarrow$ & CD-L2 $\downarrow$ &
% % F $\uparrow$ & EMD $\downarrow$ &
% % Uniformity $\downarrow$ & DCD $\downarrow$ &
% % PC CD-L1 $\downarrow$ & PC-F $\uparrow$ \\
% % \midrule
% % \multicolumn{10}{l}{\textit{(a) Unimodal point-cloud completion}} \\
% % PoinTr~\cite{pointr} & P & 12.68 & 0.79 & 0.88 & 92.42 & 0.34 & 0.52 & 11.24 & 0.91 \\
% % AnchorFormer~\cite{anchorformer} & P & 13.87 & 1.04 & 0.85 & 140.98 & 0.60 & 0.55 & 12.35 & 0.88 \\
% % SnowflakeNet~\cite{snowflakenet} & P & 11.69 & 0.78 & 0.91 & \underline{80.68} & 0.08 & 0.47 & 10.42 & 0.93 \\
% % AdaPoinTr~\cite{adapointr} & P & \underline{11.05} & \underline{0.62} & 0.92 & 90.57 & 0.14 & 0.48 & \underline{9.81} & \underline{0.94} \\
% % Unico~\cite{chen2026unico} & P & 11.28 & 0.79 & 0.91 & 88.94 & 0.10 & 0.47 & 10.35 & 0.93 \\
% % BuildAnyPoint~\cite{hua2026buildanypoint} & P & 12.88 & 1.83 & \underline{0.92} & 86.56 & \underline{0.08} & \underline{0.46} & 11.47 & 0.93 \\
% % Ours & P & \textbf{8.65} & \textbf{0.40} & \textbf{0.96} & \textbf{68.12} & \textbf{0.04} & \textbf{0.30} & \textbf{9.25} & \textbf{0.96} \\
% % \midrule
% % \multicolumn{10}{l}{\textit{(b) Multimodal completion with sparser partial observations}} \\
% % PoinTr~\cite{pointr} & P & 50.03 & 21.18 & 0.54 & 177.35 & 4.17 & 0.70 & 46.31 & 0.58 \\
% % AnchorFormer~\cite{anchorformer} & P & 49.28 & 24.25 & 0.58 & 206.22 & 0.57 & 0.69 & 45.72 & 0.61 \\
% % SnowflakeNet~\cite{snowflakenet} & P & 45.27 & 14.91 & 0.57 & 219.88 & 0.95 & 0.68 & 41.66 & 0.60 \\
% % AdaPoinTr~\cite{adapointr} & P & 58.89 & 46.25 & \underline{0.59} & 207.00 & 0.75 & \underline{0.67} & \underline{54.28} & \underline{0.62} \\
% % Unico~\cite{chen2026unico} & P & 58.42 & 43.51 & 0.55 & 172.48 & 0.12 & 0.71 & 53.61 & 0.50 \\
% % BuildAnyPoint~\cite{hua2026buildanypoint} & P & 57.20 & 20.64 & 0.36 & 166.13 & \underline{0.08} & 0.80 & 52.94 & 0.40 \\
% % \midrule
% % EGIInet~\cite{xu2024egiinet} & P+I & 44.98 & 13.45 & 0.31 & 283.07 & 1.60 & 0.95 & \underline{41.35} & \underline{0.35} \\
% % DuInNet~\cite{liu2025duinnet} & P+I & 53.76 & 17.67 & 0.26 & 294.32 & 1.55 & 0.95 & 49.82 & 0.30 \\
% % Hunyuan-Omni~\cite{hunyuan2025omni} & P+I & \underline{44.52} & \underline{10.62} & 0.30 & 145.27 & 0.27 & 0.92 & 43.15 & 0.33 \\
% % MAENet~\cite{liu2025maenet} & P+I & 46.11 & 11.08 & 0.32 & \underline{134.51} & 0.20 & 0.94 & 42.47 & 0.36 \\
% % Ours & P+I & \textbf{31.00} & \textbf{10.07} & \textbf{0.75} & \textbf{119.74} & \textbf{0.06} & \textbf{0.66} & \textbf{27.53} & \textbf{0.79} \\
% % \bottomrule
% % \end{tabular}%
% % }
% % \end{table}

% % Requires xcolor, booktabs, graphicx, and amsmath in the preamble.
% % Blue marks revised wording, headers, and corrected ranking annotations.
% % Numerical results are unchanged; columns have been reordered with their data.
% % Requires xcolor, booktabs, graphicx, and amsmath in the preamble.
% % Blue marks revised wording, headers, and corrected ranking annotations.
% % Numerical results are unchanged; columns have been reordered with their data.
% \providecommand{\rev}[1]{\textcolor{blue}{#1}}

% \begin{table}[!t]
% \centering
% \caption{\rev{\textbf{Unimodal and multimodal point-cloud completion on BuildingWorld-Image.} P: partial points; I: overhead image. Group (b) uses sparser partial observations than group (a). PC outputs precede surface generation and low-poly reconstruction; LP denotes final low-poly meshes.}}
% \label{tab:completion-combined}
% \label{tab:supp-selected}
% \label{tab:supp-multimodal}
% \footnotesize
% \setlength{\tabcolsep}{3pt}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}lccccccccc@{}}
% \toprule
% & & \multicolumn{2}{c}{\rev{Point cloud (PC)}}
% & \multicolumn{6}{c}{\rev{Low-poly mesh (LP)}} \\
% \cmidrule(lr){3-4}\cmidrule(lr){5-10}
% Method & Input
% & \rev{$\mathrm{CD}_{L_1}\downarrow$} & \rev{F-score $\uparrow$}
% & \rev{$\mathrm{CD}_{L_1}\downarrow$} & \rev{$\mathrm{CD}_{L_2}\downarrow$}
% & \rev{F-score $\uparrow$} & EMD $\downarrow$
% & \rev{Uni. $\downarrow$} & DCD $\downarrow$ \\
% \midrule
% \multicolumn{10}{l}{\textit{(a) Unimodal point-cloud completion}} \\
% PoinTr~\cite{pointr} & P & 11.24 & 0.91 & 12.68 & 0.79 & 0.88 & 92.42 & 0.34 & 0.52 \\
% AnchorFormer~\cite{anchorformer} & P & 12.35 & 0.88 & 13.87 & 1.04 & 0.85 & 140.98 & 0.60 & 0.55 \\
% SnowflakeNet~\cite{snowflakenet} & P & 10.42 & 0.93 & 11.69 & 0.78 & 0.91 & \underline{80.68} & \rev{\underline{0.08}} & 0.47 \\
% AdaPoinTr~\cite{adapointr} & P & \underline{9.81} & \underline{0.94} & \underline{11.05} & \underline{0.62} & \rev{\underline{0.92}} & 90.57 & 0.14 & 0.48 \\
% \rev{UniCo}~\cite{chen2026unico} & P & 10.35 & 0.93 & 11.28 & 0.79 & 0.91 & 88.94 & 0.10 & 0.47 \\
% BuildAnyPoint~\cite{hua2026buildanypoint} & P & 11.47 & 0.93 & 12.88 & 1.83 & \underline{0.92} & 86.56 & \underline{0.08} & \underline{0.46} \\
% Ours & P & \textbf{9.25} & \textbf{0.9625} & \textbf{8.65} & \textbf{0.40} & \textbf{0.9719} & \textbf{68.12} & \textbf{0.04} & \textbf{0.30} \\
% \midrule
% \multicolumn{10}{l}{\textit{\rev{(b) Multimodal point-cloud completion}}} \\
% PoinTr~\cite{pointr} & P & 46.31 & 0.58 & 50.03 & 21.18 & 0.54 & 177.35 & 4.17 & 0.70 \\
% AnchorFormer~\cite{anchorformer} & P & 45.72 & 0.61 & 49.28 & 24.25 & 0.58 & 206.22 & 0.57 & 0.69 \\
% SnowflakeNet~\cite{snowflakenet} & P & 41.66 & 0.60 & 45.27 & 14.91 & 0.57 & 219.88 & 0.95 & 0.68 \\
% AdaPoinTr~\cite{adapointr} & P & \rev{54.28} & \underline{0.62} & 58.89 & 46.25 & \underline{0.59} & 207.00 & 0.75 & \underline{0.67} \\
% \rev{UniCo}~\cite{chen2026unico} & P & 53.61 & 0.50 & 58.42 & 43.51 & 0.55 & 172.48 & 0.12 & 0.71 \\
% BuildAnyPoint~\cite{hua2026buildanypoint} & P & 52.94 & 0.40 & 57.20 & 20.64 & 0.36 & 166.13 & \underline{0.08} & 0.80 \\
% \midrule
% EGIInet~\cite{xu2024egiinet} & P+I & \underline{41.35} & \rev{0.55} & 44.98 & 13.45 & 0.51 & 283.07 & 1.60 & 0.95 \\
% DuInNet~\cite{liu2025duinnet} & P+I & 49.82 & 0.50 & 53.76 & 17.67 & 0.46 & 294.32 & 1.55 & 0.95 \\
% \rev{Hunyuan3D-Omni}~\cite{hunyuan2025omni} & P+I & 43.15 & 0.53 & \underline{44.52} & \underline{10.62} & 0.50 & 145.27 & 0.27 & 0.92 \\
% MAENet~\cite{liu2025maenet} & P+I & 42.47 & 0.60 & 46.11 & 11.08 & 0.52 & \underline{134.51} & 0.20 & 0.94 \\
% Ours & P+I & \textbf{27.53} & \textbf{0.7545} & \textbf{26.00} & \textbf{10.07} & \textbf{0.7741} & \textbf{119.74} & \textbf{0.06} & \textbf{0.66} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}


\providecommand{\rev}[1]{\textcolor{blue}{#1}}

\begin{table}[!t]
\centering
\caption{\rev{\textbf{Unimodal and multimodal point-cloud completion on BuildingWorld-Image.} P: partial points; I: overhead image. Group (b) uses sparser partial observations than group (a). PC outputs precede surface generation and low-poly reconstruction; LP denotes final low-poly meshes.}}
\label{tab:completion-combined}
\label{tab:supp-selected}
\label{tab:supp-multimodal}
\footnotesize
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lccccccccc@{}}
\toprule
& & \multicolumn{2}{c}{\rev{Point cloud (PC)}}
& \multicolumn{6}{c}{\rev{Low-poly mesh (LP)}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-10}
Method & Input
& \rev{$\mathrm{CD}_{L_1}\downarrow$} & \rev{F-score (\%) $\uparrow$}
& \rev{$\mathrm{CD}_{L_1}\downarrow$} & \rev{$\mathrm{CD}_{L_2}\downarrow$}
& \rev{F-score (\%) $\uparrow$} & EMD $\downarrow$
& \rev{Uni. $\downarrow$} & DCD $\downarrow$ \\
\midrule
\multicolumn{10}{l}{\textit{(a) Unimodal point-cloud completion}} \\
PoinTr~\cite{pointr} & P & 11.24 & 91.00 & 12.68 & 0.79 & 88.00 & 92.42 & 0.34 & 0.52 \\
AnchorFormer~\cite{anchorformer} & P & 12.35 & 88.00 & 13.87 & 1.04 & 85.00 & 140.98 & 0.60 & 0.55 \\
SnowflakeNet~\cite{snowflakenet} & P & 10.42 & 93.00 & 11.69 & 0.78 & 91.00 & \underline{80.68} & \rev{\underline{0.08}} & 0.47 \\
AdaPoinTr~\cite{adapointr} & P & \underline{9.81} & \underline{94.00} & \underline{11.05} & \underline{0.62} & \rev{\underline{92.00}} & 90.57 & 0.14 & 0.48 \\
\rev{UniCo}~\cite{chen2026unico} & P & 10.35 & 93.00 & 11.28 & 0.79 & 91.00 & 88.94 & 0.10 & 0.47 \\
BuildAnyPoint~\cite{hua2026buildanypoint} & P & 11.47 & 93.00 & 12.88 & 1.83 & \underline{92.00} & 86.56 & \underline{0.08} & \underline{0.46} \\
Ours & P & \textbf{9.25} & \textbf{96.25} & \textbf{8.65} & \textbf{0.40} & \textbf{97.19} & \textbf{68.12} & \textbf{0.04} & \textbf{0.30} \\
\midrule
\multicolumn{10}{l}{\textit{\rev{(b) Multimodal point-cloud completion}}} \\
PoinTr~\cite{pointr} & P & 46.31 & 58.00 & 50.03 & 21.18 & 54.00 & 177.35 & 4.17 & 0.70 \\
AnchorFormer~\cite{anchorformer} & P & 45.72 & 61.00 & 49.28 & 24.25 & 58.00 & 206.22 & 0.57 & 0.69 \\
SnowflakeNet~\cite{snowflakenet} & P & 41.66 & 60.00 & 45.27 & 14.91 & 57.00 & 219.88 & 0.95 & 0.68 \\
AdaPoinTr~\cite{adapointr} & P & \rev{54.28} & \underline{62.00} & 58.89 & 46.25 & \underline{59.00} & 207.00 & 0.75 & \underline{0.67} \\
\rev{UniCo}~\cite{chen2026unico} & P & 53.61 & 50.00 & 58.42 & 43.51 & 55.00 & 172.48 & 0.12 & 0.71 \\
BuildAnyPoint~\cite{hua2026buildanypoint} & P & 52.94 & 40.00 & 57.20 & 20.64 & 36.00 & 166.13 & \underline{0.08} & 0.80 \\
\midrule
EGIInet~\cite{xu2024egiinet} & P+I & \underline{41.35} & \rev{55.00} & 44.98 & 13.45 & 51.00 & 283.07 & 1.60 & 0.95 \\
DuInNet~\cite{liu2025duinnet} & P+I & 49.82 & 50.00 & 53.76 & 17.67 & 46.00 & 294.32 & 1.55 & 0.95 \\
\rev{Hunyuan3D-Omni}~\cite{hunyuan2025omni} & P+I & 43.15 & 53.00 & \underline{44.52} & \underline{10.62} & 50.00 & 145.27 & 0.27 & 0.92 \\
MAENet~\cite{liu2025maenet} & P+I & 42.47 & 60.00 & 46.11 & 11.08 & 52.00 & \underline{134.51} & 0.20 & 0.94 \\
Ours & P+I & \textbf{27.53} & \textbf{75.45} & \textbf{26.00} & \textbf{10.07} & \textbf{77.41} & \textbf{119.74} & \textbf{0.06} & \textbf{0.66} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/core_ablation.tex <==
% % % % \begin{table}[!t]
% % % % \centering
% % % % \renewcommand{\arraystretch}{1.0}
% % % % \caption{\textbf{Ablation of the unified generation pipeline.}
% % % % (a) Matched component variants and single-task training,
% % % % with one specialist trained for each input setting.
% % % % (b) Comparison of image-guided improvements for sparse point clouds.
% % % % (c) Surface generation and low-poly reconstruction.
% % % % The three studies use their respective evaluation cohorts.
% % % % P: points; I: image; R: coarse geometric prior.}
% % % % \label{tab:core-ablation}
% % % % \footnotesize
% % % % \setlength{\tabcolsep}{2pt}

% % % % \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc@{}}
% % % % \toprule
% % % % \multicolumn{5}{l}{
% % % %     \textit{(a) Core components: surface F@2\% $\uparrow$}
% % % % }\\
% % % % Variant & P & I & P+I & I+R\\
% % % % \midrule
% % % % \multicolumn{5}{l}{\textit{Spatial-query conditioning}}\\
% % % % condition concat
% % % % & 0.9186 & 0.5334 & 0.6071 & 0.5732\\
% % % % w/o occupancy supervision
% % % % & 0.9475 & 0.5483 & 0.7108 & 0.6403\\
% % % % w/o query read-back
% % % % & 0.9378 & 0.5117 & 0.7244 & 0.7038\\
% % % % w/o spatial prompts
% % % % & 0.9215 & 0.5147 & 0.6913 & 0.5702\\
% % % % \midrule
% % % % Single-task training
% % % % & 0.9530 & 0.5738 & 0.7291 & 0.7683\\
% % % % Full Any2Building
% % % % & \textbf{0.9625} & \textbf{0.6282}
% % % % & \textbf{0.7538} & \textbf{0.7864}\\
% % % % \bottomrule
% % % % \end{tabular*}

% % % % \par\smallskip

% % % % \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrr@{}}
% % % % \toprule
% % % % \multicolumn{5}{l}{
% % % %     \textit{(b) Image contribution: F@2\% $\uparrow$}
% % % % }\\
% % % % Degradation & Points & P & P+I & Gain\\
% % % % \midrule
% % % % None
% % % % & 4096 & 0.7439 & \textbf{0.7538} & +0.0099\\
% % % % Random
% % % % & 205 & 0.5408 & \textbf{0.7263} & +0.1855\\
% % % % Random
% % % % & 41 & 0.3867 & \textbf{0.6432} & +0.2565\\
% % % % Spatial Crop
% % % % & 41 & 0.1943 & \textbf{0.4651} & +0.2708\\
% % % % \bottomrule
% % % % \end{tabular*}

% % % % \par\smallskip

% % % % \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccccc@{}}
% % % % \toprule
% % % % \multicolumn{7}{l}{
% % % %     \textit{(c) Surface generation and low-poly reconstruction}
% % % % }\\
% % % % & \multicolumn{3}{c}{PolyFit~\cite{nan2017polyfit}}
% % % % & \multicolumn{3}{c}{RoLoPM~\cite{chen2023rolopm}}\\
% % % % \cmidrule(lr){2-4}\cmidrule(lr){5-7}
% % % % Input
% % % % & Time (s)$\downarrow$ & CD$_1\downarrow$ & F@2\%$\uparrow$
% % % % & Time (s)$\downarrow$ & CD$_1\downarrow$ & F@2\%$\uparrow$\\
% % % % \midrule
% % % % Structure
% % % % & \textbf{7.94} & 10.10 & 0.9387
% % % % & \textbf{91.20} & 9.25 & 0.9625\\
% % % % + Surface (Condition)
% % % % & 15.12 & \underline{9.21} & \underline{0.9458}
% % % % & 98.94 & \underline{8.72} & \underline{0.9706}\\
% % % % + Surface (w/o condition)
% % % % & 13.23 & \textbf{9.06} & \textbf{0.9472}
% % % % & 97.57 & \textbf{8.65} & \textbf{0.9719}\\
% % % % \bottomrule
% % % % \end{tabular*}

% % % % \end{table}

% % % \begin{table}[!t]
% % % \centering
% % % \renewcommand{\arraystretch}{1.0}
% % % \caption{\textbf{Ablation of the unified generation pipeline.}
% % % (a) Matched component variants and single-task training,
% % % with one specialist trained for each input setting.
% % % (b) Comparison of image-guided improvements for sparse point clouds.
% % % (c) Surface generation and low-poly reconstruction.
% % % The three studies use their respective evaluation cohorts.
% % % P: points; I: image; R: coarse geometric prior.}
% % % \label{tab:core-ablation}
% % % \footnotesize
% % % \setlength{\tabcolsep}{2pt}

% % % \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc@{}}
% % % \toprule
% % % \multicolumn{5}{l}{%
% % %     \textit{(a) Core components: surface F@2\% $\uparrow$}%
% % % }\\
% % % Variant & P & I & P+I & I+R\\
% % % \midrule
% % % \multicolumn{5}{l}{\textit{Spatial-query conditioning}}\\
% % % condition concat
% % % & 0.9186 & 0.5334 & 0.6071 & 0.5732\\
% % % w/o occupancy supervision
% % % & 0.9475 & 0.5483 & 0.7108 & 0.6403\\
% % % w/o query read-back
% % % & 0.9378 & 0.5117 & 0.7244 & 0.7038\\
% % % w/o spatial prompts
% % % & 0.9215 & 0.5147 & 0.6913 & 0.5702\\
% % % \midrule
% % % Single-task training
% % % & 0.9530 & 0.5738 & 0.7291 & 0.7683\\
% % % Full Any2Building
% % % & \textbf{0.9625} & \textbf{0.6282}
% % % & \textbf{0.7538} & \textbf{0.7864}\\
% % % \bottomrule
% % % \end{tabular*}

% % % \par\smallskip

% % % \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrr@{}}
% % % \toprule
% % % \multicolumn{5}{l}{%
% % %     \textit{(b) Image contribution: F@2\% $\uparrow$}%
% % % }\\
% % % Degradation & Points & P & P+I & Gain\\
% % % \midrule
% % % None
% % % & 4096 & 0.7439 & \textbf{0.7538} & +0.0099\\
% % % Random
% % % & 205 & 0.5408 & \textbf{0.7263} & +0.1855\\
% % % Random
% % % & 41 & 0.3867 & \textbf{0.6432} & +0.2565\\
% % % Spatial Crop
% % % & 41 & 0.1943 & \textbf{0.4651} & +0.2708\\
% % % \bottomrule
% % % \end{tabular*}

% % % \par\smallskip

% % % \resizebox{\linewidth}{!}{%
% % % \begin{tabular}{@{}lcccccc@{}}
% % % \toprule
% % % \multicolumn{7}{l}{%
% % %     \textit{(c) Surface generation and low-poly reconstruction}%
% % % }\\
% % % & \multicolumn{3}{c}{PolyFit~\cite{nan2017polyfit}}
% % % & \multicolumn{3}{c}{RoLoPM~\cite{chen2023rolopm}}\\
% % % \cmidrule(lr){2-4}\cmidrule(lr){5-7}
% % % Input
% % % & Time$\downarrow$ & CD$_1\downarrow$ & F@2\%$\uparrow$
% % % & Time$\downarrow$ & CD$_1\downarrow$ & F@2\%$\uparrow$\\
% % % \midrule
% % % Structure
% % % & \textbf{7.94} & 10.10 & 0.9387
% % % & \textbf{91.20} & 9.25 & 0.9625\\
% % % + Surface (Condition)
% % % & 16.12 & \underline{9.21} & \underline{0.9458}
% % % & 99.64 & \underline{8.72} & \underline{0.9706}\\
% % % + Surface (w/o condition)
% % % & 13.23 & \textbf{9.06} & \textbf{0.9472}
% % % & 97.57 & \textbf{8.65} & \textbf{0.9719}\\
% % % \bottomrule
% % % \end{tabular}%
% % % }

% % % \end{table}


% % % Requires booktabs, graphicx, and amsmath.
% % % Put this file in tables/ to match \input{tables/core_ablation}.
% % % Component/specialist rows and panel (b) retain the final-LP results
% % % confirmed by the author. Full P is updated to 0.9719 from panel (c).
% % % Full P+I and None/P+I use the author-confirmed 0.7941, which rounds
% % % to the 0.79 reported in Table 2.

% % \begin{table}[!t]
% % \centering
% % \renewcommand{\arraystretch}{1.0}
% % \caption{\textbf{Ablation of the unified generation pipeline.}
% % (a) Conditioning components and joint versus single-task training.
% % (b) Paired P and P+I inference under point degradation.
% % (c) Surface generation in the point-cloud-input setting;
% % both surface variants use predicted voxel coordinates, while
% % one additionally receives point-cloud conditioning.}
% % \label{tab:core-ablation}
% % \footnotesize
% % \setlength{\tabcolsep}{2pt}

% % \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc@{}}
% % \toprule
% % \multicolumn{5}{l}{\textit{(a) Core components: LP F@2\% $\uparrow$}}\\
% % Variant & P & I & P+I & I+R\\
% % \midrule
% % \multicolumn{5}{l}{\textit{Spatial-query conditioning}}\\
% % Condition concat & 0.9186 & 0.5334 & 0.6071 & 0.5732\\
% % w/o occupancy supervision & 0.9475 & 0.5483 & 0.7108 & 0.6403\\
% % w/o query read-back & 0.9378 & 0.5117 & 0.7244 & 0.7038\\
% % w/o spatial prompts & 0.9215 & 0.5147 & 0.6913 & 0.5702\\
% % \midrule
% % Single-task training & 0.9530 & 0.5738 & 0.7291 & 0.7683\\
% % Full Any2Building & \textbf{0.9719} & \textbf{0.6282}
% % & \textbf{0.7741} & \textbf{0.7864}\\
% % \bottomrule
% % \end{tabular*}

% % \par\smallskip

% % \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrr@{}}
% % \toprule
% % \multicolumn{5}{l}{\textit{(b) Image contribution: LP F@2\% $\uparrow$}}\\
% % Degradation & Points & P & P+I & $\Delta F$\\
% % \midrule
% % None & 4096 & 0.7439 & \textbf{0.7741} & +0.0502\\
% % Random & 205 & 0.5408 & \textbf{0.7263} & +0.1855\\
% % Random & 41 & 0.3867 & \textbf{0.6432} & +0.2565\\
% % Spatial crop & 41 & 0.1943 & \textbf{0.4651} & +0.2708\\
% % \bottomrule
% % \end{tabular*}

% % \par\smallskip

% % \resizebox{\linewidth}{!}{%
% % \begin{tabular}{@{}lcccccc@{}}
% % \toprule
% % \multicolumn{7}{l}{\textit{(c) Surface generation: final low-poly reconstruction}}\\
% % & \multicolumn{3}{c}{PolyFit~\cite{nan2017polyfit}}
% % & \multicolumn{3}{c}{RoLoPM~\cite{chen2023rolopm}}\\
% % \cmidrule(lr){2-4}\cmidrule(lr){5-7}
% % Variant
% % & Time (s)$\downarrow$ & $\mathrm{CD}_{L_1}\downarrow$ & F@2\%$\uparrow$
% % & Time (s)$\downarrow$ & $\mathrm{CD}_{L_1}\downarrow$ & F@2\%$\uparrow$\\
% % \midrule
% % Structure only
% % & \textbf{7.94} & 10.10 & 0.9387
% % & \textbf{91.20} & 9.25 & 0.9625\\
% % + Surface (w/ point cond.)
% % & 16.12 & \underline{9.21} & \underline{0.9458}
% % & 99.64 & \underline{8.72} & \underline{0.9706}\\
% % + Surface (w/o point cond.)
% % & 13.23 & \textbf{9.06} & \textbf{0.9472}
% % & 97.57 & \textbf{8.65} & \textbf{0.9719}\\
% % \bottomrule
% % \end{tabular}%
% % }

% % \end{table}
% \begin{table}[!t]
% \centering
% \renewcommand{\arraystretch}{1.0}
% \caption{\textbf{Ablation of the unified generation pipeline.}
% (a) Conditioning components and joint versus single-task training.
% (b) Paired P and P+I inference under point degradation.
% (c) Surface generation in the point-cloud-input setting;
% both surface variants use predicted voxel coordinates, while
% one additionally receives point-cloud conditioning.
% F-scores are reported as percentages.}
% \label{tab:core-ablation}
% \footnotesize
% \setlength{\tabcolsep}{2pt}

% \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc@{}}
% \toprule
% \multicolumn{5}{l}{\textit{(a) Core components: LP F@2\% $\uparrow$}}\\
% Variant & P & I & P+I & I+R\\
% \midrule
% \multicolumn{5}{l}{\textit{Spatial-query conditioning}}\\
% Condition concat & 91.86 & 53.34 & 60.71 & 57.32\\
% w/o occupancy supervision & 94.75 & 54.83 & 71.08 & 64.03\\
% w/o query read-back & 93.78 & 51.17 & 72.44 & 70.38\\
% w/o spatial prompts & 92.15 & 51.47 & 69.13 & 57.02\\
% \midrule
% Single-task training & 95.30 & 57.38 & 72.91 & 76.83\\
% Full Any2Building & \textbf{97.19} & \textbf{62.82}
% & \textbf{77.41} & \textbf{78.64}\\
% \bottomrule
% \end{tabular*}

% \par\smallskip

% \begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrr@{}}
% \toprule
% \multicolumn{5}{l}{\textit{(b) Image contribution: LP F@2\% $\uparrow$}}\\
% Degradation & Points & P & P+I & $\Delta F$ (pp)\\
% \midrule
% None & 4096 & 74.39 & \textbf{77.41} & +5.02\\
% Random & 205 & 54.08 & \textbf{72.63} & +18.55\\
% Random & 41 & 38.67 & \textbf{64.32} & +25.65\\
% Spatial crop & 41 & 19.43 & \textbf{46.51} & +27.08\\
% \bottomrule
% \end{tabular*}

% \par\smallskip

% \resizebox{\linewidth}{!}{%
% \begin{tabular}{@{}lcccccc@{}}
% \toprule
% \multicolumn{7}{l}{\textit{(c) Surface generation: final low-poly reconstruction}}\\
% & \multicolumn{3}{c}{PolyFit~\cite{nan2017polyfit}}
% & \multicolumn{3}{c}{RoLoPM~\cite{chen2023rolopm}}\\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}
% Variant
% & Time (s)$\downarrow$ & $\mathrm{CD}_{L_1}\downarrow$ & F@2\%$\uparrow$
% & Time (s)$\downarrow$ & $\mathrm{CD}_{L_1}\downarrow$ & F@2\%$\uparrow$\\
% \midrule
% Structure only
% & \textbf{7.94} & 10.10 & 93.87
% & \textbf{91.20} & 9.25 & 96.25\\
% + Surface (w/ point cond.)
% & 16.12 & \underline{9.21} & \underline{94.58}
% & 99.64 & \underline{8.72} & \underline{97.06}\\
% + Surface (w/o point cond.)
% & 13.23 & \textbf{9.06} & \textbf{94.72}
% & 97.57 & \textbf{8.65} & \textbf{97.19}\\
% \bottomrule
% \end{tabular}%
% }

% \end{table}
\begin{table}[!t]
\centering
\renewcommand{\arraystretch}{1.0}
\caption{\textbf{Ablation of the unified generation pipeline.}
(a) Conditioning components and joint versus single-task training.
(b) Paired P and P+I inference under point degradation.
(c) Surface generation in the point-cloud-input setting;
both surface variants use predicted voxel coordinates, while
one additionally receives point-cloud conditioning.
F-scores are reported as percentages.}
\label{tab:core-ablation}
\footnotesize
\setlength{\tabcolsep}{2pt}

\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccc@{}}
\toprule
\multicolumn{5}{l}{\textit{(a) Core components: LP F@2\% $\uparrow$}}\\
Variant & P & I & P+I & I+R\\
\midrule
\multicolumn{5}{l}{\textit{Spatial-query conditioning}}\\
Condition concat & 91.86 & 53.34 & 60.71 & 57.32\\
w/o occupancy supervision & 94.75 & 54.83 & 71.08 & 64.03\\
w/o query read-back & 93.78 & 51.17 & 72.44 & 70.38\\
w/o spatial prompts & 92.15 & 51.47 & 69.13 & 57.02\\
\midrule
Single-task training & 95.30 & 57.38 & 72.91 & 76.83\\
Full Any2Building & \textbf{97.19} & \textbf{62.82}
& \textbf{77.41} & \textbf{78.64}\\
\bottomrule
\end{tabular*}

\par\smallskip

\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lrrrr@{}}
\toprule
\multicolumn{5}{l}{\textit{(b) Image contribution: LP F@2\% $\uparrow$}}\\
Degradation & Points & P & P+I & $\Delta F$ (pp)\\
\midrule
None & 4096 & 74.39 & \textbf{77.41} & +5.02\\
Random & 205 & 54.08 & \textbf{72.63} & +18.55\\
Random & 41 & 38.67 & \textbf{64.32} & +25.65\\
Spatial crop & 41 & 19.43 & \textbf{46.51} & +27.08\\
\bottomrule
\end{tabular*}

\par\smallskip

\resizebox{\linewidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multicolumn{7}{l}{\textit{(c) Surface generation: final low-poly reconstruction}}\\
& \multicolumn{3}{c}{PolyFit~\cite{nan2017polyfit}}
& \multicolumn{3}{c}{RoLoPM~\cite{chen2023rolopm}}\\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Variant
& Time (s)$\downarrow$ & $\mathrm{CD}_{L_1}\downarrow$ & F@2\%$\uparrow$
& Time (s)$\downarrow$ & $\mathrm{CD}_{L_1}\downarrow$ & F@2\%$\uparrow$\\
\midrule
Structure only
& \textbf{7.94} & 10.10 & 93.87
& \textbf{91.20} & 9.25 & 96.25\\
+ Surface (w/ point cond.)
& 16.12 & \underline{9.21} & \underline{94.58}
& 99.64 & \underline{8.72} & \underline{97.06}\\
+ Surface (w/o point cond.)
& 13.23 & \textbf{9.06} & \textbf{94.72}
& 97.57 & \textbf{8.65} & \textbf{97.19}\\
\bottomrule
\end{tabular}%
}

\end{table}

==> tables/dataset_cities.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Training data pool.} Geometry counts unique city-qualified BuildingWorld low-poly building targets. Image counts targets with a corresponding remote-sensing image and low-poly building mesh, after quality filtering within the fixed training split and without tier quotas. Image is a subset of Geometry; the columns are not additive. Counts refer to paired targets, not augmented views.}
\label{tab:dataset-cities}
\small\setlength{\tabcolsep}{5pt}
\begin{tabular}{lrr}
\toprule
City & Geometry & Image\\
\midrule
Boston & 167,410 & 63,857 \\
Calgary & 322,649 & 224,190 \\
Cambridge & 17,041 & 11,191 \\
Cape Town & 274,598 & 125,202 \\
Edmonton & 370,673 & 246,540 \\
Greater Geelong & 886 & 596 \\
Hong Kong & 25,544 & 11,724 \\
Melbourne & 8,909 & 5,895 \\
Mississauga & 145,080 & 139,489 \\
Montreal & 24,866 & 24,652 \\
New York & 47,815 & 44,370 \\
Perth & 4,111 & 3,843 \\
Philadelphia & 2,907 & 2,117 \\
San Francisco & 91,359 & 65,583 \\
Tokyo & 34,507 & 10,998 \\
Toronto & 4,255 & 4,197 \\
Wellington & 15,213 & 13,165 \\
Yarra & 25,201 & 13,587 \\
\midrule
Total & 1,583,024 & 1,011,196\\
\bottomrule
\end{tabular}
\end{table}

==> tables/image_gain.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Visual evidence complements missing geometry.} Surface F@2\% on 64 held-out Berlin buildings. Each row pairs the same points and noise with/without imagery. Table~\ref{tab:supp-image-gain} reports the full sweep.}
\label{tab:supp-image-gain-compact}
\small\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrr}
\toprule
Degradation & Points & P & P+I & Gain\\
\midrule
None & 4096 & 0.8647 & \textbf{0.8745} & +0.0099\\
Random & 819 & 0.8274 & \textbf{0.8687} & +0.0413\\
Random & 205 & 0.6408 & \textbf{0.8263} & +0.1855\\
Random & 41 & 0.3867 & \textbf{0.6432} & +0.2565\\
\midrule
Spatial & 819 & 0.5573 & \textbf{0.7334} & +0.1761\\
Spatial & 205 & 0.3872 & \textbf{0.5708} & +0.1837\\
Spatial & 41 & 0.1943 & \textbf{0.4651} & +0.2707\\
\bottomrule
\end{tabular}
\end{table}


==> tables/image_gain_full.tex <==
\begin{table}[t]
\centering
\begin{threeparttable}
\caption{Image contribution under point-cloud degradation on
64 Berlin cases outside the training list.
F-scores are evaluated at a distance threshold of 0.02
after Stage2.}
\label{tab:supp-image-gain}
\small\setlength{\tabcolsep}{3pt}
\begin{tabular}{lrccc}
\toprule
Degradation
& Points
& P $\uparrow$
& P+I $\uparrow$
& Gain $\uparrow$ \\
\midrule
None
& 4096 & 0.8647 & \textbf{0.8745} & +0.0099 \\
\midrule
Random thinning
& 2048 & 0.8526 & \textbf{0.8754} & +0.0228 \\
Random thinning
& 819  & 0.8274 & \textbf{0.8687} & +0.0413 \\
Random thinning
& 410  & 0.7547 & \textbf{0.8563} & +0.1015 \\
Random thinning
& 205  & 0.6408 & \textbf{0.8263} & +0.1855 \\
Random thinning
& 41   & 0.3867 & \textbf{0.6432} & +0.2565 \\
\midrule
Spatial drop
& 2048 & 0.7215 & \textbf{0.8186} & +0.0970 \\
Spatial drop
& 819  & 0.5573 & \textbf{0.7334} & +0.1761 \\
Spatial drop
& 410  & 0.4665 & \textbf{0.6642} & +0.1977 \\
Spatial drop
& 205  & 0.3872 & \textbf{0.5708} & +0.1837 \\
Spatial drop
& 41   & 0.1943 & \textbf{0.4651} & +0.2707 \\
\bottomrule
\end{tabular}
\begin{tablenotes}[flushleft]
\footnotesize
\item \textit{Notes:}
PC denotes point cloud. For each case and degradation
setting, both input configurations use the same retained
point cloud and noise realization. Points reports
the actual number of input points.
Gain is the absolute F-score improvement from adding images.
All values are reported as fractions.
Bold indicates the higher F-score within each row.
Gains are reproduced as supplied and may differ slightly
from differences computed using the rounded F-scores.
\end{tablenotes}
\end{threeparttable}
\end{table}


==> tables/image_generation.tex <==
% \begin{table}[!t]
% \centering
% \caption{\textbf{Image-based building generation.}
% I: Image; R: coarse prior.
% Metric definitions and evaluation protocols follow Table~2.
% $^{\dagger}$PSNR and SSIM compare matched four-view renderings of
% predicted and reference textured meshes.}
% \label{tab:image-generation}
% \footnotesize
% \setlength{\tabcolsep}{2pt}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{@{}lcrrrrrrrr@{}}
% \toprule
% Method & Input
% & CD$_1\downarrow$ & CD$_2\downarrow$ & F$\uparrow$
% & EMD$\downarrow$ & U$\downarrow$ & DCD$\downarrow$
% & PSNR$^{\dagger}\uparrow$ & SSIM$^{\dagger}\uparrow$ \\
% \midrule
% \multicolumn{10}{l}{\textit{(c) Single-image generation from real remote-sensing instance images with background}} \\
% TRELLIS~\cite{xiang2025trellis} & I
% & \underline{54.89} & 9.14 & \underline{0.49}
% & \underline{111.08} & \underline{0.03} & \underline{0.66}
% & \underline{10.91} & 0.26 \\
% TRELLIS.2~\cite{xiang2025trellis2} & I
% & 65.09 & 9.90 & 0.31
% & 124.57 & 0.03 & 0.79
% & 10.80 & \underline{0.28} \\
% SAM 3D~\cite{sam3d2025} & I
% & 55.82 & \underline{8.53} & 0.44
% & 117.59 & 0.04 & 0.71
% & 9.26 & 0.23 \\
% Ours & I
% & \textbf{38.90} & \textbf{6.32} & \textbf{0.62}
% & \textbf{93.16} & \textbf{0.03} & \textbf{0.60}
% & \textbf{12.63} & \textbf{0.34} \\
% \midrule
% \multicolumn{10}{l}{\textit{(d) Orthophoto setting: prior-assisted generation}} \\
% SpaceControl~\cite{fedele2026spacecontrol} & I+R
% & 34.77 & 3.83 & \underline{0.61}
% & 86.15 & \textbf{0.02} & 0.57
% & \underline{11.65} & \underline{0.30} \\
% Hunyuan-Omni~\cite{hunyuan2025omni} & I+R
% & \underline{32.46} & 3.51 & 0.60
% & \underline{83.27} & 0.04 & \underline{0.55}
% & 11.38 & 0.29 \\
% SatSkylines~\cite{jin2026satskylines} & I+R
% & 33.12 & \underline{3.42} & 0.59
% & 84.69 & 0.05 & 0.56
% & 11.21 & 0.28 \\
% Ours & I+R
% & \textbf{17.23} & \textbf{1.53} & \textbf{0.79}
% & \textbf{57.82} & \underline{0.03} & \textbf{0.37}
% & \textbf{14.05} & \textbf{0.41} \\
% \bottomrule
% \end{tabular}%
% }
% \end{table}


% Requires xcolor, booktabs, graphicx, and amsmath in the preamble.
% Blue marks revised wording, headers, and corrected ranking annotations.
% Numerical results are unchanged; columns have been reordered with their data.
% Requires xcolor, booktabs, graphicx, and amsmath in the preamble.
% Blue marks revised wording, headers, and corrected ranking annotations.
% Numerical results are unchanged; columns have been reordered with their data.
\providecommand{\rev}[1]{\textcolor{blue}{#1}}

\begin{table}[!t]
\centering
\caption{\rev{\textbf{Image-based building generation on BuildingWorld-Image.} I: overhead image; R: coarse geometric prior. Backgrounds are retained in (a) and removed in (b). PSNR and SSIM compare matched four-view renderings of predicted and reference textured meshes.}}
\label{tab:image-generation}
\footnotesize
\setlength{\tabcolsep}{2pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}lcrrrrrrrr@{}}
\toprule
& & \multicolumn{6}{c}{\rev{Geometry}}
& \multicolumn{2}{c}{\rev{Appearance}} \\
\cmidrule(lr){3-8}\cmidrule(lr){9-10}
Method & Input
& \rev{$\mathrm{CD}_{L_1}\downarrow$} & \rev{$\mathrm{CD}_{L_2}\downarrow$}
& \rev{F-score $\uparrow$} & EMD $\downarrow$
& \rev{Uni. $\downarrow$} & DCD $\downarrow$
& \rev{PSNR (dB) $\uparrow$} & \rev{SSIM $\uparrow$} \\
\midrule
\multicolumn{10}{l}{\textit{\rev{(a) Single-image generation}}} \\
TRELLIS~\cite{xiang2025trellis} & I & \underline{54.89} & 9.14 & \underline{49.20} & \underline{111.08} & \rev{\textbf{0.03}} & \underline{0.66} & \underline{10.91} & 0.26 \\
TRELLIS.2~\cite{xiang2025trellis2} & I & 65.09 & 9.90 & 31.05 & 124.57 & \rev{\textbf{0.03}} & 0.79 & 10.80 & \underline{0.28} \\
SAM 3D~\cite{sam3d2025} & I & 55.82 & \underline{8.53} & 44.34 & 117.59 & \rev{\underline{0.04}} & 0.71 & 9.26 & 0.23 \\
Ours & I & \textbf{38.90} & \textbf{6.32} & \textbf{62.82} & \textbf{93.16} & \textbf{0.03} & \textbf{0.60} & \textbf{12.63} & \textbf{0.34} \\
\midrule
\multicolumn{10}{l}{\textit{\rev{(b) Prior-assisted generation}}} \\
SpaceControl~\cite{fedele2026spacecontrol} & I+R & 34.77 & 3.83 & \underline{61.93} & 86.15 & \textbf{0.02} & 0.57 & \underline{11.65} & \underline{0.30} \\
\rev{Hunyuan3D-Omni}~\cite{hunyuan2025omni} & I+R & \underline{32.46} & 3.51 & 60.82 & \underline{83.27} & 0.04 & \underline{0.55} & 11.38 & 0.29 \\
SatSkylines~\cite{jin2026satskylines} & I+R & 33.12 & \underline{3.42} & 59.62 & 84.69 & 0.05 & 0.56 & 11.21 & 0.28 \\
Ours & I+R & \textbf{17.23} & \textbf{1.53} & \textbf{78.64} & \textbf{57.82} & \underline{0.03} & \textbf{0.37} & \textbf{14.05} & \textbf{0.41} \\
\bottomrule
\end{tabular}%
}
\end{table}


==> tables/lowpoly_full_inline.tex <==
\begin{table}[t]
\centering
\caption{Low-poly reconstruction (arithmetic means).
CD denotes symmetric Chamfer-L1 $\times 10^3$;
F-score uses a 2\% distance threshold.
Full time includes recorded network inference and low-poly conversion;
evaluation alignment is excluded.
Best results are bold; second-best results are underlined.}
\label{tab:supp-lowpoly}
\small
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.12}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|rrr|rrr@{}}
\toprule
& \multicolumn{3}{c|}{PolyFit}
& \multicolumn{3}{c}{RoLoPM} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Method
& Full time (s)$\downarrow$ & CD$\downarrow$ & F-score$\uparrow$
& Full time (s)$\downarrow$ & CD$\downarrow$ & F-score$\uparrow$ \\
\midrule
FoldingNet~\cite{foldingnet}
& 121.29 & 48.02 & 0.42
& 239.08 & 51.76 & 0.31 \\
PCN~\cite{pcn}
& 116.92 & 55.86 & 0.33
& 219.13 & 56.53 & 0.38 \\
TopNet~\cite{topnet}$^{\ddagger}$
& 217.59 & 87.90 & 0.09
& 382.77 & 64.25 & 0.21 \\
GRNet~\cite{grnet}
& 125.69 & 70.88 & 0.33
& 215.34 & 54.77 & 0.30 \\
SnowflakeNet~\cite{snowflakenet}
& 62.57 & 55.98 & 0.47
& 186.02 & 11.69 & 0.91 \\
PoinTr~\cite{pointr}
& 73.33 & 42.55 & 0.44
& 204.71 & 12.68 & 0.88 \\
AnchorFormer~\cite{anchorformer}
& 61.12 & 51.11 & 0.49
& 167.30 & 13.87 & 0.85 \\
AdaPoinTr~\cite{adapointr}
& 60.91 & 40.14 & 0.52
& 161.57 & 11.05 & 0.92 \\
BuildAnyPoint~\cite{hua2026buildanypoint}$^{\dagger}$
& 38.39 & 12.88 & 0.92
& \textbf{38.39} & 12.88 & 0.92 \\
\midrule
Ours (Stage1)
& \textbf{7.94} & \underline{10.10} & \underline{0.93}
& \underline{91.20} & \underline{9.25} & \underline{0.96} \\
Ours (Stage1 + Stage2)
& \underline{13.23} & \textbf{9.06} & \textbf{0.94}
& 97.57 & \textbf{8.65} & \textbf{0.97} \\
\bottomrule
\end{tabular}%
}
\par\vspace{2pt}
\begin{minipage}{\columnwidth}
\footnotesize
All methods except BuildAnyPoint use common settings within
each conversion backend; input-specific adapters are described
in the text.
$^{\dagger}$BuildAnyPoint uses its native completion and mesh decoder.
$^{\ddagger}$PolyFit succeeds on half of the TopNet outputs:
failures receive zero F-score, CD is computed only over
successful outputs, and time includes all attempts.
Full time aggregates cached GPU inference and measured CPU
conversion using eight cores, rather than a new end-to-end
wall-clock measurement. Untimed initialization, I/O,
cleanup/export, and metric computation are excluded.
\end{minipage}
\end{table}
